An Efficient, Reliable and Observable Collective Communication Library in Large-scale GPU Training Clusters

Large-scale LLM training requires collective communication libraries to exchange data among distributed GPUs. As a company dedicated to building and operating large-scale GPU training clusters, we encounter several practical limitations of NCCL in production, including 1) SM competition between computation and communication, 2) expensive restart costs under link failures, and 3) insufficient observability of transient collective communication anomalies. To address these challenges, we propose VCCL, an efficient, reliable, and observable collective communication library in large-scale GPU training clusters. VCCL removes SM-consuming P2P kernels by moving intra-node data movement and stream dependency enforcement to CPU threads and GPU copy engines. VCCL also introduces a primary-backup QP mechanism to tolerate frequent NIC port failures, and designs a window-based monitor to observe network anomalies at O({\mu}s) level. We opensource VCCL and deploy it in production training clusters for several months. Compared with NCCL, VCCL improves training throughput by up to 5.28% and reduces massive GPU resource wastage through runtime fault tolerance and finegrained monitor. We also share experience and lessons we learned during the deployment of VCCL in large-scale clusters.

==> texfiles/4evaluation_1.tex <==
\begin{figure}[t]
  \centering
  \subfigure[Inter-node P2P bandwidth.]
  {\vspace{-1.5\baselineskip} \includegraphics[width=0.48\linewidth]{figure/plot/inter_bandwidth.pdf}}
  \subfigure[Inter-node P2P latency.]{\vspace{-1.5\baselineskip} \includegraphics[width=0.48\linewidth]{figure/plot/inter_latency.pdf}} 
  \\
  \subfigure[Intra-node P2P bandwidth.]{\vspace{-1.5\baselineskip} \includegraphics[width=0.48\linewidth]{figure/plot/intra_bandwidth.pdf}}
  \subfigure[Intra-node P2P latency.]{\vspace{-1.5\baselineskip} \includegraphics[width=0.48\linewidth]{figure/plot/intra_latency.pdf}}
  \vspace{-1\baselineskip}
  \caption{Bandwidth and latency performance.}
  \label{fig-p2p-performance}
  \vspace{-1\baselineskip}
\end{figure}

\begin{figure*}[t]
  \centering
  \subfigure[384 GPUs-176B.]{\includegraphics[width=0.24\linewidth]{figure/plot/training_384-176B.pdf}}
  \subfigure[576 GPUs-176B.]{\includegraphics[width=0.24\linewidth]{figure/plot/training_384-176B.pdf}}
  \subfigure[768 GPUs-176B.]{\includegraphics[width=0.24\linewidth]{figure/plot/training_384-176B.pdf}}
  \subfigure[960 GPUs-176B.]{\includegraphics[width=0.24\linewidth]{figure/plot/training_384-176B.pdf}}
  \\
  \subfigure[256 GPUs-314B.]{\includegraphics[width=0.24\linewidth]{figure/plot/training_384-176B.pdf}}
  \subfigure[512 GPUs-314B.]{\includegraphics[width=0.24\linewidth]{figure/plot/training_384-176B.pdf}}
  \subfigure[768 GPUs-314B.]{\includegraphics[width=0.24\linewidth]{figure/plot/training_384-176B.pdf}}
  \subfigure[1024 GPUs-314B.]{\includegraphics[width=0.24\linewidth]{figure/plot/training_384-176B.pdf}}
  \vspace{-1\baselineskip}
  \caption{Training performance of \X.}
  \label{fig-smfree-training-performance}
  \vspace{-1\baselineskip}
\end{figure*}

%\begin{table}[t]
%    \caption{Kernel invocation and SM consumption.}
%    \centering
%    \footnotesize
%    \renewcommand{\arraystretch}{1.1}
%    \vspace{-1\baselineskip}
%    \begin{tabular}{|c|l|c|}
%    \hline
%     & \multicolumn{1}{c|}{Operations (percentage)} & SM utilization \\ \hline
%    \multirow{5}{*}{NCCL} & \texttt{ncclDevKernel\_SendRecv} (68.8\%) & \multirow{5}{*}{3.2\%} \\ \cline{2-2}
%    & \texttt{verifyPrepare} (27.0\%) &  \\ \cline{2-2}
%     & \texttt{prepareInput2} (3.5\%) &  \\ \cline{2-2}
%     & {[}CUDA memset{]} (0.4\%) &  \\ \cline{2-2}
%     & {[}CUDA memcpy Host-to-Device{]} (0.4\%) &  \\ \hline
%    \multirow{4}{*}{\X} & \texttt{verifyPrepare} (86.1\%) & \multirow{4}{*}{2.8\%} \\ \cline{2-2}
%     & \texttt{prepareInput2} (11.4\%) &  \\ \cline{2-2}
%     & {[}CUDA memset{]} (1.3\%) &  \\ \cline{2-2}
%     & {[}CUDA memcpy Host-to-Device{]} (1.2\%) &  \\ \hline
%    \end{tabular}
%    \label{tab-sm}
%    \vspace{-1\baselineskip}
%\end{table}

% \vspace{-0.5\baselineskip}
\section{Evaluation}
\label{sec-eval}

Based on NCCL v2.26.6, we implement \X with 7,000 lines of C codes, \zmh{which is publicly available at Github \cite{vccl-github}.}
We evaluate \X in three dimensions:
1) how efficient is \X's SM-free P2P design to improve CC performance and overlaps in PP (\S\ref{subsec-eval-efficiency})?
2) how reliable is \X's primary-backup QP mechanism to tolerate RNIC port downs (\S\ref{subsec-eval-fault-tolerance})?
3) how observable is \X's monitor to perceive transient CC's network anomalies (\S\ref{subsec-eval-monitor})?
% 4) how feasible is \X to enable heterogeneous CC and training within a multi-vendor GPU cluster (\S\ref{subsec-eval-generality})?

\vspace{-0.5\baselineskip}
\subsection{Experimental Setups}
\label{subsec-eval-setup}

\noindent\textbf{Cluster environment.}
% We conduct experiments in our testing cluster, which is composed of:
To avoid interfering with LLM training, we conduct experiments on the subset of servers in a production cluster, including:
% The cluster is composed of:
% 1) GPUs manufactured by different vendors, including NVIDIA H100 \cite{h100} \& A800 \cite{a800}, MetaX C550 \cite{metax} and Iluvatar BI-V100 \cite{iluvatar};
1) 1024 NVIDIA Hopper GPUs; %\cite{h200};
% , and 32 other GPUs from vendor A and vendor B;
2) NVIDIA ConnectX-7 RNICs \cite{cx7} and BlueField-3 DPU \cite{bf3datasheet}.
% 3) switches produced by Cisco and Huawei.
Each server is equipped with 8 homogeneous GPUs and 9 RNICs, and they are connected with a 1:1 oversubscribed two-layer CLOS topology network with 400Gbps bandwidth.

\noindent\textbf{Workloads and baseline.}
% We use Llama 3 \cite{grattafiori2024llama}, an open-source dense LLM with sizes of 6B (small), 32B (medium) and 70B (large) as the training workload.
% We use \zmh{GPT-2 \cite{radford2019language}, an open-source dense LLM} with sizes of 6B, 32B, 70B and 175B as the default training workload, \czt{as well as Qwen-xxx \cite{yang2024qwen2} sized at xxx to evaluate the generality of \X.}
We use GPT-2 \cite{radford2019language}, an open-source dense LLM with different sizes of 6B, 32B, 70B, 177B and 314B as the training workloads.
To perform large-scale distributed training, we integrate \X into Megatron-LM \cite{megatronlm} with 3D parallelism.
We also use NCCL-Tests \cite{nccltest} to generate some typical CC workloads, and Nsight \cite{nsight} to visualize the runtime kernel invocation and SM utilization.
As for baseline, we compare \X with NCCL v2.26.6 and NCCLX \cite{si2025ncclx} in terms of training throughput in Tera Floating Point Operations Per Second (TFLOPS), algorithm bandwidth in GB/s, and system overhead.
To ensure a fair comparison, we explicitly implement the zero-copy mechanism for the NCCL baseline.
The training hyperparameters and default settings are listed in Table \ref{tab-hyperparameter} in Supplemental Material \ref{appendix-experiment-settings}.

% \noindent\textbf{Baseline.}
% We integrate \X into Megatron-LM to prove the feasibility of each design, and compare with NCCL in terms of training throughput (i.e., Tera Floating Point Operations Per Second (TFLOPS) and Tokens per GPU per Second (TGS)), algorithm bandwidth in GB/s and system overhead.
% The default settings of \X and NCCL are listed in Table \ref{tab-default-setting}.

% \begin{table}[t]
%     \caption{SM utilization of NCCL and \X.}
%     \centering
%     \footnotesize
%     \vspace{-1\baselineskip}
%     \setlength{\tabcolsep}{1.5mm}{
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%      \diagbox[width=9em]{SM util.}{Workload} & \begin{tabular}[c]{@{}c@{}}Intra-host\\ P2P\end{tabular} & \begin{tabular}[c]{@{}c@{}}Inter-node\\ P2P\end{tabular} & \begin{tabular}[c]{@{}c@{}}8$\times$8\\ \texttt{alltoall}\end{tabular} & \begin{tabular}[c]{@{}c@{}}16$\times$16\\ \texttt{alltoall}\end{tabular} \\ \hline
%     NCCL & 23.1 & 3.2 & 24.7 & 3.1 \\ \hline
%     \X & 14.3 & 2.1 & 12.5 & \czt{8.3} \\ \hline
%     \end{tabular}
%     }
%     \label{tab-nccl-sm}
%     \vspace{-2\baselineskip}
% \end{table}

% \begin{figure*}[t]
%   \centering
%   \subfigure[SM utilization.]{\includegraphics[width=0.24\linewidth]{figure/plot/kernel_free_sm.pdf}}
%   \subfigure[Inter-node P2P performance.]{\includegraphics[width=0.24\linewidth]{figure/plot/kernel_free_p2p_bandwidth.pdf}}
%   \subfigure[\texttt{alltoall} performance.]{\includegraphics[width=0.24\linewidth]{figure/plot/kernel_free_alltoall_bandwidth.pdf}}
%   \subfigure[Training performance.]{\includegraphics[width=0.24\linewidth]{figure/plot/kernel_free_tflops.pdf}}
%   \vspace{-1\baselineskip}
%   \caption{Zero-copy P2P.}
%   \label{fig-kernel-free-eval}
%   \vspace{-1.5\baselineskip}
% \end{figure*}


% \begin{figure}[t]
%   \centering
%   \subfigure[\czt{NCCL.}]{\includegraphics[width=0.45\textwidth]{figure/plot/sm_vccl.png}}
%   \subfigure[\X.]{\includegraphics[width=0.45\textwidth]{figure/plot/sm_vccl.png}}
%   \vspace{-1\baselineskip}
%   \caption{SM consumption of \texttt{send/recv}.}
%   \label{fig-p2p-sm}
%   \vspace{-0.5\baselineskip}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\vspace{-0.5\baselineskip}
\subsection{Efficiency}
\label{subsec-eval-efficiency}

\noindent\textbf{P2P performance.}
Figure \ref{fig-p2p-performance} compares the P2P performance of \texttt{send/recv} workloads generated by NCCL-Tests.
%For bandwidth performance, as we increase the message size in Figure \ref{fig-p2p-performance}(a), \X's algorithm bandwidth outperforms NCCL by at least 20.12\% when the message size is 1GB.
For inter-node P2P, since \X and NCCL are both free of cumbersome buffer copies, they achieve similar bandwidth for large messages (> 8MB).
% This is because CPUs, equipped with fewer but stronger computing units for general computation tasks, exhibit higher capability to process P2P communication than GPUs designed for simple and parallel computation.
%This is because the zero-copy design of \X eliminates the frequent and consuming memory copies from the application buffer to the chunk buffer with User Buffer Registration.
%Meanwhile, since \X completely eliminates the GPU-CPU synchronization, \X's latency outperforms NCCL by the average of 18.9\% for small messages.
Meanwhile, \X reduces small-message latency by 18.9\% on average by eliminating GPU-CPU synchronization.
%For intra-node P2P, we see a different results.
%As can be seen, for large size messages, \X's bandwidth performance achieves about 7\% improvement than NCCL.
For intra-node P2P, \X improves large-message bandwidth by approximately 7\%.
The reason behind is that its copy-engine-based approach issues wider transactions that better saturate NVLink compared to SM-based transfers.
However, we also observe higher latency for small intra-node messages — a result of contention for limited copy-engine resources — this is not a critical bottleneck in production environments. 
In PP, message sizes typically exceed 32MB, rendering small-message latency overhead negligible. 
Furthermore, the primary value of VCCL’s SM-free mechanism lies in eliminating SM contention, which maximizes the potential for computation-communication overlap. Consequently, the bandwidth efficiency and SM availability gains far outweigh the minor latency penalties for small P2P messages.
% due to limited copy-engine resources.
%However, since the data communication between PP is typically large, at least about 32MB and the ultimate goal of SM-free P2P is for eliminating the SM competition, we only discuss it in \S \ref{sec-discussion}.
% Fortunately, since PP typically involves transfers exceeding 32MB, and the primary goal of \X's SM-free mechanism is to eliminate SM contention, we only discuss it in \S \ref{sec-discussion}.
%For latency performance, we also notice that \X achieves at least 28.5\% lower P2P latency than NCCL when the message size is small.
%The reason is that in addition to the elimination of buffer copies, CPU offloading reduces the signal synchronization between GPUs and CPUs, whose overhead can dominate the entire process of P2P primitives especially with small messages.
%Therefore, the results prove \X's feasibility and efficiency to deliver better P2P performance with SM-free design for both large and small message sizes.

\noindent\textbf{Training performance.}
We present the training performance of different LLMs and GPU numbers, with \X integrated into Megatron-LM to enable overlap between forward \& backward passes and \texttt{send/recv} operations during PP.
%For training accuracy, Figure \ref{fig-training-loss} shows that \X exhibits the same loss value trend as NCCL for GPT-2 in different sizes, proving that \X's SM-free P2P design using \texttt{waitValue} guarantees the correct interaction and order between computation and communication as kernels do in NCCL.
\zmh{For training throughput, as Figure \ref{fig-smfree-training-performance} shows, \X achieves about 490 TFLOPS averagely in different model sizes and GPU numbers, which outperforms NCCL's training throughput by at most 6.02\%.}
The reasons are two-fold.
Firstly, \X not only empowers overlap between computation and communication during PP, but also improves P2P bandwidth with zero memory copies for faster synchronization for activations and gradients among GPU workers.
Secondly, the offloading mechanism with SM-free P2P ensures more SM resources can be allocated to computation tasks for faster forward \& backward passes.
The results validate that \X's zero-copy and SM-free P2P designs both contribute to the improvement of overall training performance.
Meanwhile, we conduct extensive training experiments to compare the loss convergence between NCCL and \X (details in Supplemental Material \ref{appendix-loss-value}), demonstrating that \X’s SM-free design does not affect training behavior.


\noindent\textbf{Resource consumption.}
We profile the SM and CPU resources consumption of \X and NCCL, indicating that \X successfully eliminates GPU kernel launches for communication, while introducing only about 2\% additional CPU utilization (details can be seen in Supplemental Material \ref{appendix-resource-consumption}).
%Table \ref{tab-sm} shows the kernel invocation and SM utilization of inter-host P2P communication using NCCL and \X.
%The second column in the table represents the invoked kernels and their respective percentage of executing duration, which are collected by Nsight.
%Obviously, NCCL invokes a \texttt{send/recv} kernel \texttt{ncclDevKernel\_SendRecv} to perform the reduction-free P2P communication, which accounts for 68.3\% execution time and 3.2\% SM usage.
%Instead, except for two inevitable NCCL-Tests kernels (i.e., \texttt{prepareInput2} for data preparation and \texttt{verifyPrepare} for result verification), \X does not launch any GPU kernels to perform the P2P communication, thereby consuming lower SM utilization than NCCL.
%Note that in practical LLM training, \texttt{prepareInput2} and \texttt{verifyPrepare} will not be invoked, such that \X's SM-free P2P can achieve almost zero SM consumption, which can be scheduled in computation to accelerate the LLM training process.
% Especially, to saturate much higher intra-node interconnection than inter-node bandwidth, NCCL has to consume 7.71$\times$ more SM resources for higher throughput.
% , but instead migrates the communication burden from GPUs to CPUs, thereby occupying no GPU resources for reduction-free primitives.
%As shown in Table \ref{tab-sm} in Supplemental Material \ref{appendix-resource-consumption}, NCCL relies on the \texttt{ncclDevKernel\_SendRecv} kernel for P2P communication, consuming 68.3\% of the execution time and 3.2\% of SM resources. 
%In contrast, \X eliminates GPU kernel launches for data transfer (excluding computational kernels). 
%By achieving SM-free P2P communication, \X allows the GPU to dedicate all SM resources to computation, thereby accelerating the overall LLM training process.


%Figure \ref{fig-kernelfree-cpu} in Supplemental Material \ref{appendix-resource-consumption} compares the CPU utilization of a GPU server using NCCL and \X, respectively.
%Although \X's SM-free design offloads P2P from GPU kernels to CPU proxies, it only introduces about 2\% more CPU utilization than NCCL.
%The result validates \X's deployability and feasibility in real-world GPU cluster, where a low CPU utilization is essential to maintain the CC efficiency (discussed in \S\ref{sec-discussion}).




%\begin{figure}[t]
%  \centering
%  \subfigure[177B model.]{\includegraphics[width=0.49\linewidth]{figure/plot/tflops_176b.pdf}}
%  \subfigure[314B model]{\includegraphics[width=0.49\linewidth]{figure/plot/tflops_314b.pdf}}
%  \vspace{-1\baselineskip}
%  \caption{Training throughput.}
%  \label{fig-training-tflops}
%  \vspace{-1.5\baselineskip}
%\end{figure}

\vspace{-0.5\baselineskip}
\subsection{Reliability}
\label{subsec-eval-fault-tolerance}



%\begin{figure}[t]
%    \includegraphics[width=0.99\linewidth]{figure/plot/fault_tolerance_training.pdf}
 %   \centering
 %   \vspace{-1\baselineskip}
%    \caption{Training performance of fault tolerance.}
%    \label{fig-fault-tolerance-training}
%    \vspace{-1\baselineskip}
%\end{figure}

\noindent\textbf{Tolerance to link failures.}
%To evaluate fault tolerance, we manually bring down a specific RNIC port from 4s to 19s, whose failed duration exceeds the default retry timeout, and bring up the RNIC port at 19s again.
%Figure \ref{fig-primary-back-qp-eval}(a) compares the runtime bandwidth of NCCL and \X with \texttt{allreduce} and \texttt{reducescatter} workloads.
To evaluate the reliability of \X, we select two representative communication workloads: \texttt{Send\allowbreak Recv} (primitive for pipeline parallelism) and \texttt{All\allowbreak Reduce} (widely used in tensor and data parallelism).
Figure \ref{fig-primary-back-qp-eval}(a) depicts the runtime bandwidth of \X under a link failure.
Specifically, we manually bring down a RNIC port from 4s to 19s, whose failed duration exceeds the default retry timeout, and bring up the RNIC port at 19s again.
The red area denotes the retry period, and yellow area denotes \X is transmitting using the backup QP, while green area denotes \X switches back to the primary QP when the RNIC port is up again.
When a port down occurs, \X spend about 10s to reconnect, staying at 0GB/s during the retry period.
%After retry timeout, NCCL terminates the connection and the entire CC, failing to resume the communication due to the lack of fault tolerance.
%In contrast, after 10s retry, \X switches to the backup QP using another RNIC port in good condition, and for \texttt{allreduce} and \texttt{reducescatter} workloads, \X resumes 76.6\% and 58.1\% bandwidth of primary QP's performance, respectively.
After 10s retry, \X switches to the backup QP using an alternative healthy RNIC port, ensuring in-place communication recovery. 
Additionally, when the RNIC port is brought up again, \X can switch back to the primary QP and deliver the ideal bandwidth.
Meanwhile, to evaluate the resilience of \X against multi-port failures, we perform an \texttt{AllReduce} stress test, where detailed results are provided in Supplemental Material \ref{appendix-multi-port-failures}.

\begin{figure}[t]
  \centering
  \subfigure[Single-port failures.]{\includegraphics[width=0.49\linewidth]{figure/plot/fault_tolerance_single_port_3.pdf}}
  \subfigure[Training performance.]{\includegraphics[width=0.49\linewidth, trim=5pt 0 5pt 0, clip]{figure/plot/fault_tolerance_training.pdf}}
  \vspace{-1\baselineskip}
  \caption{Tolerance to link failures.}
  \label{fig-primary-back-qp-eval}
  \vspace{-1\baselineskip}
\end{figure}

\noindent\textbf{Training throughput.}
%Figure \ref{fig-fault-tolerance-training} presents the training throughput when fault tolerance is triggered to use the backup QP for transmission during training a 70B model.
%When the RNIC port fails, \X's backup QP still delivers a comparable training throughput as the normal scenario using the primary QP, with TFLOPS only declines by 0.38\% at most.
%It proves that our primary-backup QP mechanism can tolerate RNIC port failure and maintain a reliable training even with failure.
Figure \ref{fig-primary-back-qp-eval}(b) compares the training throughput of \X and NCCL when handling link failures during the training of a 70B model. 
While both systems experience temporary stalls during minor link flaps, NCCL inevitably hangs when facing severe link failures that exceed hardware retransmission limits. 
In contrast, \X leverages its primary-backup QP mechanism to recover training after a timeout, with TFLOPS almost remaining constant. 
The red region represents the significant GPU hours \X reclaims. 
In large-scale production deployments, where link failures requiring manual intervention are increasingly frequent, \X’s ability to maintain continuity offers substantial savings in computational resources and operational overhead.

% \begin{figure}[t]
%     \includegraphics[width=0.99\linewidth]{figure/plot/telemetry_accuracy.pdf}
%     \centering
%     \vspace{-0.5\baselineskip}
%     \caption{Accuracy and overhead.}
%     \label{fig-telemetry-accuracy-overhead}
%     \vspace{-1.5\baselineskip}
% \end{figure}

\begin{figure}[t]
    \includegraphics[width=0.99\linewidth]{figure/plot/telemetry_throughput.pdf}
    \centering
    \vspace{-1\baselineskip}
    \caption{Monitor results with different window sizes.}
    \label{fig-telemetry-throughput}
    \vspace{-1.2\baselineskip}
\end{figure}

% \begin{figure}[t]
%   \centering
%   \subfigure[\czt{Runtime throughput}]{\includegraphics[width=0.99\linewidth]{figure/plot/telemetry_throughput.pdf}}
%   \subfigure[Monitor accuracy]{\includegraphics[width=0.49\linewidth]{figure/plot/telemetry_accuracy.pdf}}
%   \subfigure[Monitor overhead]{\includegraphics[width=0.49\linewidth]{figure/plot/telemetry_overhead.pdf}}
%   \vspace{-0.5\baselineskip}
%   \caption{Window-based anomaly monitor.}
%   \label{fig-telemetry-eval}
%   \vspace{-1\baselineskip}
% \end{figure}

%\vspace{-1\baselineskip}
\subsection{Observability}
\label{subsec-eval-monitor}
%\vspace{-0.5\baselineskip}

\noindent\textbf{Monitoring accuracy with sliding window.}
To evaluate the observability, we generate a background P2P workload between a pair of servers, and insert a disturbance traffic to compete for bandwidth, making the background workload converge to a lower and stable throughput.
Figure \ref{fig-telemetry-throughput} presents the runtime throughput in a 10$\mu$s granularity with different window sizes.
Especially, when window size is 1, it equals to the naive per-message scheme.
% When the disturbance workload starts at 100$\mu$s, \X can monitor the throughput drop within 10$\mu$s timescale, empowering \X to be aware of transient anomaly of collective communication.
We notice \X can capture the transient $O(\mu s)$ throughput changes, but shows a very fluctuating measuring result with per-message scheme.
With a large window size of 32, \X can smooth out the fluctuation and reflects more accurate results closer to the ground truth, but fails to perceive the instantaneous changes.
For example, when disturbance traffic arrives at 100$\mu$s, per-message scheme shows an intense fluctuation, but a large window size directly drops to the new converged throughput.
Therefore, we set the window size as 8 to achieve the tradeoff between measuring accuracy and fluctuation sensitivity in our environment.

% \noindent\textbf{Monitoring accuracy.}
% We evaluate the effects of sliding window's size on the monitoring accuracy.
% Note that when the window size is 1, it is equivalent to the naive per-WR scheme illustrated in Figure \ref{fig-verb-estimation}(a).
% To evaluate the accuracy under each window size, we use Mean Squared Error (MSE) to calculate the error by $\frac{1}{n}\sum_{i = 1}^{n}{(x_i-\overline{x})^2}$, where $x_i$ is the measured throughput at each time point, and $\overline{x}$ is the \czt{ground truth throughput obtained by RNIC counters.}
% Figure \ref{fig-telemetry-eval}(b) demonstrates the logarithmic MSE values in different window sizes.
% When the size increases from 1 to 32, the measuring error exhibits an obvious decline, but if we increase the window size from 32 to 128, the measuring error rises correspondingly.
% The results validate the relationship between measuring accuracy and window size discussed in \S\ref{subsec-eval-monitor}.

\begin{figure}[t]
  \centering
  \subfigure[Normal.]{\includegraphics[width=0.49\linewidth, trim=20pt 0 45pt 0, clip]{figure/plot/telemetry_pinpoint_case1_line_8.pdf}}%
  \subfigure[Manual shutdown.]{\includegraphics[width=0.49\linewidth, trim=45pt 0 20pt 0, clip]{figure/plot/telemetry_pinpoint_case2_line8.pdf}}%
  \\
  \vspace{-1\baselineskip}
  \subfigure[Background traffic.]{\includegraphics[width=0.49\linewidth, trim=20pt 0 45pt 0, clip]{figure/plot/telemetry_pinpoint_case3_line11.pdf}}%
  \subfigure[Background computation.]{\includegraphics[width=0.49\linewidth, trim=45pt 0 20pt 0, clip]{figure/plot/telemetry_pinpoint_case4_line8.pdf}}%
  \vspace{-1\baselineskip}
  \caption{Network performance tracing of CC across four representative cases.}
  \label{fig-pinpoint}
  \vspace{-1.5\baselineskip}
\end{figure}

\noindent\textbf{Pinpointing network straggler.}
%Figure ? demonstrates the effectiveness of our heuristical pinpointing algorithm.
Figure \ref{fig-pinpoint} illustrates the effectiveness of \X’s heuristic pinpointing algorithm across four representative scenarios: 
(1) a normal CC task, 
(2) the manual termination of a CC task, 
(3) a CC task under network interference (small-packet perftest), and 
(4) a CC task under transient hardware interference (GPU-burn). 
As shown in the results, the normal case (case 1) maintains stable \texttt{bandwidth} and \texttt{remain\allowbreak To\allowbreak Send} (\texttt{RTS}), indicating a healthy state. 
%In case 2, the \texttt{bandwidth} decline at the tail is correctly identified as normal behavior, as it stems from the exhaustion of the NIC’s data buffer rather than network anomaly. 
In case 2, \X correctly classifies the terminal bandwidth decline as normal behavior, attributing it to the exhaustion of the NIC’s data buffer rather than a network anomaly.
Crucially, \X distinguishes between network and non-network issues: in case 3, the simultaneous drop in \texttt{bandwidth} and \texttt{RTS} accumulation allows \X to pinpoint a network anomaly; conversely, in case 4, despite the significant \texttt{bandwidth} drop caused by GPU resource contention, the absence of data accumulation on the NIC prevents a false positive. 
%These experimental data demonstrate that \X can accurately localize network-layer anomalies while remaining resilient to other-point performance fluctuations.
These results underscore \X’s ability to accurately localize network stragglers while remaining resilient to other performance fluctuations.


\noindent\textbf{System overhead.}
As shown in Table \ref{tab-monitor-overhead} in Supplemental Material \ref{appendix-resource-consumption}, we evaluate the system overhead of our window-based monitor in terms of CPU and memory.
Generally, it does not incur much consumption on CPU and memory, both of which are still far from reaching their capacity limits.
%This proves the efficiency of \X's monitor, which is a feasible approach not affecting training performance in real-world training systems (discussed in \S\ref{sec-operating}).

% \begin{figure}[t]
%   \centering
%   \subfigure[P2P performance]{\includegraphics[width=0.49\linewidth]{figure/plot/hetero_p2p.pdf}}
%   \subfigure[\czt{Training performance}]{\includegraphics[width=0.49\linewidth]{figure/plot/hetero_tflops.pdf}}
%   \vspace{-0.5\baselineskip}
%   \caption{Multi-vendor collectives.}
%   \label{fig-multi-vendor-collective}
%   \vspace{-1\baselineskip}
% \end{figure}

% \subsection{Heterogeneity}
% \label{subsec-eval-generality}

% \begin{figure}[t]
%     \includegraphics[width=0.99\linewidth]{figure/plot/hetero_p2p_v2.pdf}
%     \centering
%     \vspace{-1\baselineskip}
%     \caption{P2P performance.}
%     \label{fig-multi-vendor-collective}
%     \vspace{-0.5\baselineskip}
% \end{figure}

% \begin{table}[t]
%     \caption{Training with multi-vendor GPUs.}
%     \centering
%     \footnotesize
%     \vspace{-0.5\baselineskip}
%     \begin{tabular}{|c|>{\centering\arraybackslash}p{1.3cm}|c|}
%     \hline
%     \diagbox[width=11.8em]{GPUs}{Metrics} & TGS & \begin{tabular}[c]{@{}c@{}}Loss after\\ 50 iterations\end{tabular} \\ \hline
%     32 NVIDIA H100 GPUs & 850 & 12 $\rightarrow$ 7.318 \\ \hline
%     \begin{tabular}[c]{@{}c@{}}16 NVIDIA H100 GPUs +\\ 16 Vendor B's GPUs\end{tabular} & 602 & 12 $\rightarrow$ 7.301 \\ \hline
%     \end{tabular}
%     \label{tab-multi-vendor-training}
%     \vspace{-1\baselineskip}
% \end{table}

% \noindent\textbf{P2P performance.}
% We evaluate the inter-node P2P performance of three pairs of GPUs with varying message sizes.
% The first pair is two homogeneous NVIDIA A800 GPUs.
% The second pair is two homogeneous vendor A's GPUs.
% The third heterogeneous pair includes an NVIDIA A800 GPU and a vendor A's GPU.
% % To enable P2P communication between two GPUs, \X follows the procedure of Figure \ref{fig-heterogeneous}(a) that executes xCCL interfaces for the homogeneous pair, and invokes \X P2P interface for the heterogeneous pair.
% As shown in Figure \ref{fig-heterogeneous}, \X enables the P2P communication among two heterogeneous GPUs, which also outperforms the second pair of vendor A's GPUs with lower communicating throughput.
% Additionally, when the message is smaller than 128KB, the heterogeneous pair can achieve almost the same performance as the homogeneous NVIDIA pair.
% As message size increases, the largest gap between the heterogeneous pair and the NVIDIA pair is smaller than 5GB/s, which is still tolerable in dense model training that are not sensitive to CC bandwidth (discussed in \S\ref{sec-operating}).
% The results prove that \X supports heterogeneous P2P and allows NVIDIA GPUs to compensate for the wimpy communication of other vendors' GPUs.

% \noindent\textbf{Training performance.}
% We also evaluate the LLM training performance with two sets of GPUs.
% The first homogeneous set is 32 NVIDIA H100 GPUs, while the second heterogeneous set includes 16 NVIDIA H100 GPUs and 16 Vendor B's GPUs.
% We train a 70B model and evaluate their training throughput and precision after 50 iterations.
% As shown in Table \ref{tab-multi-vendor-training}, the loss values of heterogeneous and homogeneous sets both drop from 12 to about 7.3, proving the training precision can be guaranteed in a multi-vendor environment.
% Meanwhile, TGS performance of heterogeneous set achieves 29.1\% lower than the NVIDIA homogeneous set.
% Considering the significant price differential between NVIDIA and vendor B, we note their training throughput gap is acceptable.
% Therefore, \X offers a technically feasible and budget-friendly approach for customers to save the infrastructure costs.


==> texfiles/5deployment_1.tex <==
% \vspace{-0.5\baselineskip}
\section{Deployment: \X in production}
\label{sec-deployment}

%We deploy \X in large-scale GPU clusters of our customers, and it has been operating stably for several months.
%Here we share our operating experiences in running \X in real-world environment, and hope our experiences and lessons can help developers build a better CC service in production-level LLM training clusters.
\X was initially deployed in a 2k-GPU cluster in December 2023, and has since been integrated into all our subsequent delivery clusters, scaling up to 24k GPUs.
To protect our customer's privacy, specific institution identities are omitted.
Originally, \X was developed for customized optimizations, like topology-aware channel reconstruction or enhanced NIC selection in dual-port environments.
Since NCCL has introduced similar capabilities during evolution, we only focus on the deployment of \X regarding the newly proposed features.
Notably, the statistics showed in this section are collected at the cluster level rather than the individual task level for privacy.

\noindent\textbf{Full-stack trouble shooting with \X.}
In large-scale GPU training, reliability is more crucial than efficiency since failures or stragglers cause training performance slowdown or even crash of the whole process, leading to great GPU wastage.
%Therefore, it is essential to provide full-stack trouble shooting system for quicker faulty localization.
%Figure \ref{fig:trouble_shooting} shows our full-stack trouble shooting system for large-scale training clusters.
To address this, we propose a full-stack troubleshooting system with \X designed for fault localization and recovery.
Figure \ref{fig:trouble_shooting} in Supplemental Material \ref{appendix-full-stack-troubleshooting} illustrates the system architecture, which is organized into three hierarchical layers:
%1) Object Layer (Bottom): This layer targets both physical and logical resources, extending from underlying hardware (e.g., GPUs, network fabrics, storage) to cloud-native platforms and applications. 
1) Object Layer: covers both physical and logical resources, from hardware (e.g., GPUs, network, storage) to cloud platforms and applications, enabling end-to-end observability.
%Such full-stack coverage provides the comprehensive visibility needed for effective fault diagnosis.
2) Monitoring and Acquisition Layer (Middle): bridges resources and decisions via specialized collectors.
%While standard tools (e.g., dcgmi \cite{dcgmi} for GPUs, Prometheus \cite{prometheus} for K8s) handle general metrics, we integrate \X to address the specific challenges of distributed training networks. 
%Unlike traditional coarse-grained monitoring (e.g., SNMP \cite{SNMP}), \X provides NIC-level troubleshooting and O(us) monitoring capabilities. 
%This high-resolution telemetry is critical for capturing transient network jitters and collective communication bottlenecks that are invisible to second-level sampling.
Standard tools (e.g., dcgmi \cite{dcgmi}, Prometheus\cite{prometheus}) handle general metrics, while \X provides NIC-level troubleshooting and O(us) monitoring capabilities, capturing transient network jitters and collective communication bottlenecks that are invisible to coarse-grained approaches (e.g., SNMP \cite{SNMP}).
%Furthermore, \X supports customizable application-level metrics for our different customers, such as \texttt{opFuncTimes} and \texttt{ccType}.
\X also supports customizable application-level metrics (e.g., \texttt{opFuncTimes}, \texttt{ccType}).
3) Decision and Interaction Layer (Top): an intelligent agent aggregates multi-dimensional data via Elastic stacks \cite{elasticGithub} and platform APIs, driving visualization, alerting, ticketing, and automated fault isolation.
Figure \ref{fig-production-troubleshooting} shows that, with our full-stack troubleshooting platfrom, the runtime diagnosis percentage gradually approaches \zmj{XXX\%}.

%For clusters operating at scale, manual debugging is infeasible. 
%This platform transforms troubleshooting from a reactive process into a proactive, automated system. 
%This platform enables proactive, automated troubleshooting by correlating fine-grained network telemetry to accurately identify stragglers and root cause.
%By correlating \X's online network performance monitor, the system can precisely pinpoint "straggler" nodes or subtle link degradations, enabling rapid isolation of faulty components to maximize training efficiency and cluster utilization.
%Our production deployment confirms that VCCL detects port exception and issues alerts in a near-instantaneous manner.

\noindent\textbf{The necessity of link failure tolerance.}
Empowered by the comprehensive full-stack diagnostic platform, we can accurately identify the root causes of $95\%$ training anomalies within 30 seconds.
However, a significant gap remains between fault localization and manual intervention by site reliability engineers. 
Figure \ref{fig-production-fault-tolerance} illustrates the impact of link failures within a production cluster of 24K GPUs.
Prior to June 2025, the cluster utilize a single-plane topology where link failures resulted in massive GPU-hour wastage. 
While the transition to a dual-plane architecture in June 2025 reduce about \zmj{XXX\%} idle GPU time, standard NIC bonding still proves insufficient for mitigating link failures within a single plane environment.
%Prior to September 2025—before the integration of the fault tolerance features in \X—monthly GPU time wastage reached as high as \zmj{XXX} GPU-hours due to network instability. 
%Following the deployment of \X’s fault-tolerant mechanisms, we observed a \zmj{XXX\%} reduction in idle GPU resources. 
The subsequent deployment of \X's fault tolerance feature successfully addresses this issue, leading to a \zmj{XXX\%} reduction in idle GPU resources.
This substantial decrease in computational overhead underscores the critical necessity of runtime link-failure tolerance in large-scale distributed training clusters.

\begin{figure}[t]
  \centering
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/plot/production_fault_tolerance.pdf}
    \vspace{-2\baselineskip}
    \captionof{figure}{Runtime diagnosis percentage.}
    \label{fig-production-troubleshooting}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/plot/production_fault_tolerance.pdf}
    \vspace{-2\baselineskip}
    \captionof{figure}{GPU idle time caused by link failures.}
    \label{fig-production-fault-tolerance}
  \end{minipage}
  \vspace{-1.5\baselineskip}
\end{figure}

%We deep dive into NCCL's memory allocation design and identify two primary sources of this inefficiency:
%(1) NCCL pre-allocates resources for all three protocols (SIMPLE, LL, LL128) and multiple channels to maximize NVLINK/Network utilization. 
%However, this approach often leads to resource over-provisioning, as typical training workloads rarely utilize all protocols or the full channel capacity simultaneously.
%Additionally, NCCL allocates 2MB per channel to satisfy CUDA virtual memory management granularity.
%This approach often leads to resource over-provisioning, as typical training workloads rarely utilize all protocols or the full channel capacity simultaneously.
%(1) NCCL aggressively pre-allocates resources for all protocols (SIMPLE, LL, LL128) and channels with 2 MiB alignment, despite most workloads utilizing only a subset.
%2) NCCL requires intermediate send/recv buffers on the GPU for intra-node data movement.
%Meanwhile, NCCL proposes registered buffer feature \cite{nccl_registered_buffer} in version 2.28.9, which gives opportunities to achieve zero-copy communication. 
%This motivates us to investigate whether the registered buffer feature can be leveraged to further eliminate unnecessary memory overhead.

\noindent\textbf{Optimizing memory usage of \X.}
%Our customers had complained about the unexpected high GPU memory consumption of NCCL for a long time.
%To be worse, we found that for specific MoE models (e.g., Qwen3-235B \cite{qwen3235b}), NCCL may consume up to 10GB High-Bandwidth Memory (HBM), which severely constrains model parallelism strategies.
During the deployment of \X, we observe unexpected high GPU memory consumption, reaching 10GB High-Bandwidth Memory (HBM) for specific MoE models (e.g., Qwen3-235B \cite{qwen3235b}).
This inefficiency, which severely constrains model parallelism strategies, stems from NCCL's default aggressive pre-allocation across all protocols and channels, as well as its reliance on intermediate GPU buffers for intra-node data movement.
To mitigate this, \X introduces a dynamic memory pool design.
First, \X adopts a lazy allocation strategy, where resources are assigned to connections only upon their first runtime usage. 
The system maintains a 2MiB-aligned memory pool to allocate minimal necessary memory for each peer, dynamically expanding via \texttt{cuCallocAsync} when the pool is exhausted. 
Second, by leveraging zero-copy mechanisms for both intra-node and inter-node P2P primitives, we are allowed to eliminate intermediate buffers, thereby minimizing the memory footprint.
Compared with NCCL, \X achieves about \zmj{10\%} memory reduction in practical deployments of models with complex parallelism.


